Lifetime Difference and CP-Violating Phase in the B_s^0 System

From an analysis of the decay Bs -> J/psi phi we obtain the width difference between the light and heavy mass eigenstates, and the CP-violating phase.

==> list_of_visitor_addresses_r2.tex <==
% list_of_visitor_addresses_r2.tex                            1/5/07
%
%
\bibitem[*]{alton}
Visitor from Augustana College, Sioux Falls, SD, USA
\bibitem[\S]{podesta-lerma}
Visitor from ICN-UNAM, Mexico City, Mexico.
%\bibitem[\dag]{kozminski}
%Visitor from Lewis University, Romeoville, IL, USA
\bibitem[\ddag]{voutilainen}
Visitor from Helsinki Institute of Physics, Helsinki, Finland.
\bibitem[\#]{wenger}
Visitor from Universit{\"a}t Z{\"u}rich, Z{\"u}rich, Switzerland.
%
\vskip 0.25cm

